Multimodal Image Denoising based on Coupled Dictionary Learning

In this paper, we propose a new multimodal image denoising approach to attenuate white Gaussian additive noise in a given image modality under the aid of a guidance image modality. The proposed coupled image denoising approach consists of two stages: coupled sparse coding and reconstruction. The first stage performs joint sparse transform for multimodal images with respect to a group of learned coupled dictionaries, followed by a shrinkage operation on the sparse representations. Then, in the second stage, the shrunken representations, together with coupled dictionaries, contribute to the reconstruction of the denoised image via an inverse transform. The proposed denoising scheme demonstrates the capability to capture both the common and distinct features of different data modalities. This capability makes our approach more robust to inconsistencies between the guidance and the target images, thereby overcoming drawbacks such as the texture copying artifacts. Experiments on real multimodal images demonstrate that the proposed approach is able to better employ guidance information to bring notable benefits in the image denoising task with respect to the state-of-the-art.

==> Appendices_V2.tex <==
%\addcontentsline{toc}{chapter}{Appendices}

%\renewcommand{\appendixname}{Appendix~\Alph{section}}
%\appendix
%\appendixpage


%
%%This appendix gives more details about the derivation and experiments results.
%\section*{Appendix A: CDLMRI}
%
%We provide more details in relation to Section \ref{ssec:CDLMRI} CDLMRI in this appendix.
%
%%\subsection*{2.2 CDLMRI}
%
%
%\mypar{Stage 1) Coupled Dictionary Learning (details)}
%The dictionary update step is to solve the optimization problem:
%\begin{equation} \label{Eq:CDLMRI_DictUpdateStep}
%\small
%\begin{array}{cl}
%\underset{
%	\begin{subarray}{c}
%	\boldsymbol{\Psi}_c, \boldsymbol{\Psi}, \boldsymbol{\Phi}_c, \boldsymbol{\Phi} \\
%	\end{subarray}
%}{\text{minimize}}
%&  \!\!\!\!		
%\sum\limits_{ij} 
%\Big\{
%\| \mathbf{R}_{ij} \mathbf{x}^{(1)} - ( \boldsymbol{\Psi}_c \mathbf{z}_{ij} + \boldsymbol{\Psi} \mathbf{u}_{ij} ) \|_2^2 
%\\
%&  \!\!\!\!
%\quad \;
%+
%\| \mathbf{R}_{ij} \mathbf{x}^{(2)} - ( \boldsymbol{\Phi}_c \mathbf{z}_{ij} + \boldsymbol{\Phi} \mathbf{v}_{ij} ) \|_2^2 
%\Big\}
%\\
%\text{subject to}
%& \!\!\!\!
%\left\| \begin{bmatrix}
%\boldsymbol{\psi}_{ck} \\ \boldsymbol{\phi}_{ck} 
%\end{bmatrix} \right\|_2^2 \leq 1, 
%\|\boldsymbol{\psi}_k \|_2^2 \leq 1, 
%\|\boldsymbol{\phi}_k \|_2^2 \leq 1, 
%\, \forall k % = 1,2, \ldots, K\,,
%\end{array}
%\end{equation}
%\noindent
%Given a subset of the patches to constitute the training dataset $\mathbf{X}^{(1)}=[\cdots, \mathbf{x}_{ij}^{(1)}, \cdots]$ and $\mathbf{X}^{(2)}=[\cdots, \mathbf{x}_{ij}^{(2)}, \cdots]$ in Stage 1), the optimization problem~\eqref{Eq:CDLMRI_DictUpdateStep} is equivalent to:
%\begin{equation*} 
%\small
%\begin{array}{cl}
%\underset{
%	\begin{subarray}{c}
%	\boldsymbol{\Psi}_c, \boldsymbol{\Psi}, \boldsymbol{\Phi}_c, \boldsymbol{\Phi} \\
%	\end{subarray}
%}{\text{minimize}}
%&  \!\!\!\!		
%\left\|
%\begin{bmatrix} 
%\mathbf{X}^{(1)} - \boldsymbol{\Psi} \mathbf{U} \\ 
%\mathbf{X}^{(2)} -  \boldsymbol{\Phi} \mathbf{V}
%\end{bmatrix} 
%- 	
%\begin{bmatrix} 
%\boldsymbol{\Psi}_c \\ 
%\boldsymbol{\Phi}_c
%\end{bmatrix} 
%\mathbf{Z} \right\|_F^2
%\\
%\text{subject to}
%& \!\!\!\!
%\left\| \begin{bmatrix}
%\boldsymbol{\psi}_{ck} \\ \boldsymbol{\phi}_{ck} 
%\end{bmatrix} \right\|_2^2 \leq 1, 
%\|\boldsymbol{\psi}_k \|_2^2 \leq 1, 
%\|\boldsymbol{\phi}_k \|_2^2 \leq 1, 
%\, \forall k % = 1,2, \ldots, K\,,
%\end{array}
%\end{equation*}
%\noindent
%where, $\mathbf{Z}=[\cdots, \mathbf{z}_{ij}^{(1)}, \cdots]$, $\mathbf{U}=[\cdots, \mathbf{u}_{ij}^{(1)}, \cdots]$, $\mathbf{V}=[\cdots, \mathbf{v}_{ij}^{(1)}, \cdots]$. Taking the dictionary update of $\boldsymbol{\Psi}_c$ and $\boldsymbol{\Phi}_c$ for example, we update the atom pairs one by one. For the $k$-th atom pair $\boldsymbol{\psi}_c$ and $\boldsymbol{\phi}_c$, we can immediately establish that
%\begin{equation*} 
%\small
%\begin{array}{rl}
%\mathbf{d}_k \leftarrow
%\underset{
%	\begin{subarray}{c}
%	\mathbf{d} \\
%	\end{subarray}
%}{\text{min}}
%&  \!\!\!\!		
%\left\|
%\begin{bmatrix} 
%\mathbf{X}^{(1)} - \boldsymbol{\Psi} \mathbf{U} \\ 
%\mathbf{X}^{(2)} -  \boldsymbol{\Phi} \mathbf{V}
%\end{bmatrix} 
%- 	
%\begin{bmatrix} 
%\boldsymbol{\Psi}_c \\ 
%\boldsymbol{\Phi}_c
%\end{bmatrix} 
%\mathbf{Z} 
%+
%\begin{bmatrix}
%\boldsymbol{\psi}_{ck}  \\
%\boldsymbol{\phi}_{ck}  \\
%\end{bmatrix}
%\mathbf{z}^k
%-
%\mathbf{d} \mathbf{z}^k
%\right\|_F^2
%\\
%\text{s.t.}
%& \!\!\!\!
%\left\| \mathbf{d} \right\|_2^2 \leq 1, 
%\end{array}
%\end{equation*}
%\noindent
%By expanding the Frobenius norm and removing the constant term, it turns out that the above problem is equivalent to the optimization problem
%\begin{equation*} 
%\small
%\begin{array}{rl}
%%\mathbf{d}_k \leftarrow
%\underset{
%	\begin{subarray}{c}
%	\mathbf{d} \\
%	\end{subarray}
%}{\text{min}}
%&  \!\!\!\!	
%\frac{1}{2}
%\left\|
%\mathbf{d} \mathbf{z}^k
%\right\|_F^2	
%- \mathbf{d}^T
%\left(
%\begin{bmatrix} 
%\mathbf{X}^{(1)} - \boldsymbol{\Psi} \mathbf{U} \\ 
%\mathbf{X}^{(2)} -  \boldsymbol{\Phi} \mathbf{V}
%\end{bmatrix} 
%- 	
%\begin{bmatrix} 
%\boldsymbol{\Psi}_c \\ 
%\boldsymbol{\Phi}_c
%\end{bmatrix} 
%\mathbf{Z} 
%+
%\begin{bmatrix}
%\boldsymbol{\psi}_{ck}  \\
%\boldsymbol{\phi}_{ck}  \\
%\end{bmatrix}
%\mathbf{z}^k
%\right) 
%\mathbf{z}^{k^T}
%\\
%\text{s.t.}
%& \!\!\!\!
%\left\| \mathbf{d} \right\|_2^2 \leq 1, 
%\end{array}
%\end{equation*}
%where $\mathbf{z}^k$ denotes the $k$-th row of $\mathbf{Z}$.\footnote{Note that $\mathbf{z}^k$ is a row vector resulting from the derivative w.r.t the $k$-th atom pair, while $\mathbf{z}_{ij}$ is a column vector corresponding to the $ij$-th patch pair.}
%%
%\noindent
%We compute the derivative of the objective w.r.t. $\mathbf{d}$, leading to a norm equation:
%\begin{align*}
%&
%\mathbf{d}_k  
%\leftarrow \frac{1}{\mathbf{z}^k {\mathbf{z}^k}^T}
%%			 (\widetilde{\mathbf{X}} 
%\left(
%\begin{bmatrix} 
%\mathbf{X}^{(1)} - \boldsymbol{\Psi} \mathbf{U} \\ 
%\mathbf{X}^{(2)} -  \boldsymbol{\Phi} \mathbf{V}
%\end{bmatrix} 
%- 	
%\begin{bmatrix} 
%\boldsymbol{\Psi}_c \\ 
%\boldsymbol{\Phi}_c
%\end{bmatrix} 
%\mathbf{Z} \right)
%{\mathbf{z}^k}^T + 
%\begin{bmatrix}
%\boldsymbol{\psi}_{ck}  \\
%\boldsymbol{\phi}_{ck}  \\
%\end{bmatrix}
%\end{align*}
%\noindent
%Then, we apply the $\ell_2$ norm constraint. 
%\begin{align*}
%&
%\begin{bmatrix}
%\boldsymbol{\psi}_{ck}  \\
%\boldsymbol{\phi}_{ck}  \\
%\end{bmatrix}
%= \mathbf{d}_k \leftarrow \frac{\mathbf{d}_k}{\max(\|\mathbf{d}_k \|_2, 1)} 
%%			; \forall k=1,\cdots, K.
%\end{align*}
%The dictionary update of $\boldsymbol{\Psi}$ and $\boldsymbol{\Phi}$ is performed in a similar way. In order to accelerate the training, the proposed algorithm can be updated to online training version without difficulty.




\mypar{Appendix: More Experiments}
% Introduction to T1 and T2 characteristics.

In this appendix, we provide more experiment results for demonstration of our algorithm.

%\section{Experiments}
%\label{sec:Experiments}
%\vspace{-0.2cm}

%
%% Training images
\begin{figure*}[bhtp]
	\centering
	% ------------------------------------------- 
	%	\begin{minipage}[b]{0.06\linewidth}
	%		\centering
	%		{\footnotesize Infrared} \hfill % \vfill
	%		{\footnotesize RGB}
	%	\end{minipage} 
	\begin{minipage}[b]{0.1\linewidth}
		\centering
		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-0.png}
		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-1.png}
	\end{minipage} 
	\begin{minipage}[b]{0.1\linewidth}
		\centering
		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-2.png}
		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-3.png}
	\end{minipage} 
	\begin{minipage}[b]{0.1\linewidth}
		\centering
		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-4.png}
		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-5.png}
	\end{minipage} 
	\begin{minipage}[b]{0.1\linewidth}
		\centering
		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-6.png}
		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-7.png}
	\end{minipage} 
	\begin{minipage}[b]{0.1\linewidth}
		\centering
		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-8.png}
		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-9.png}
	\end{minipage} 
	\begin{minipage}[b]{0.1\linewidth}
		\centering
		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-10.png}
		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-11.png}
	\end{minipage} 
	\begin{minipage}[b]{0.1\linewidth}
		\centering
		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-12.png}
		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-13.png}
	\end{minipage} 
	\begin{minipage}[b]{0.1\linewidth}
		\centering
		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-14.png}
		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-15.png}
	\end{minipage} 
	\begin{minipage}[b]{0.1\linewidth}
		\centering
		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-16.png}
		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-17.png}
	\end{minipage} 
	\\
	% ------------------------------------------- 
	% ------------------------------------------- 
	%	\begin{minipage}[b]{0.06\linewidth}
	%		\centering	{\phantom{{\footnotesize Methods}}} 
	%	\end{minipage}
	%	\begin{minipage}[b]{0.15\linewidth}
	%		\centering	{\footnotesize $\sigma=4$}
	%	\end{minipage} 
	% -------------------------------------------	
	\caption{Some training infrared/RGB image pairs. The first row represents the infrared images and the second row represents the corresponding RGB images.}
	\label{Fig:TrainIms}
\end{figure*}
%
%
%% Testing images
\begin{figure*}[bhtp]
	\centering
	% ------------------------------------------- 
	%	\begin{minipage}[b]{0.06\linewidth}
	%		\centering
	%		{\footnotesize Infrared} \hfill % \vfill
	%		{\footnotesize RGB}
	%	\end{minipage} 
	\begin{minipage}[b]{0.11\linewidth}
		\centering
		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-0.png}
		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-1.png}
	\end{minipage} 
	\begin{minipage}[b]{0.11\linewidth}
		\centering
		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-2.png}
		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-3.png}
	\end{minipage} 
	\begin{minipage}[b]{0.11\linewidth}
		\centering
		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-4.png}
		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-5.png}
	\end{minipage} 
	\begin{minipage}[b]{0.11\linewidth}
		\centering
		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-6.png}
		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-7.png}
	\end{minipage} 
	\begin{minipage}[b]{0.11\linewidth}
		\centering
		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-8.png}
		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-9.png}
	\end{minipage} 
	\begin{minipage}[b]{0.11\linewidth}
		\centering
		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-10.png}
		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-11.png}
	\end{minipage} 
	\begin{minipage}[b]{0.11\linewidth}
		\centering
		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-12.png}
		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-13.png}
	\end{minipage} 
	\begin{minipage}[b]{0.11\linewidth}
		\centering
		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-14.png}
		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-15.png}
	\end{minipage} 
	\\
	% ------------------------------------------- 
	\begin{minipage}[b]{0.11\linewidth}
		\centering {\footnotesize urban 0004}
	\end{minipage} 
	\begin{minipage}[b]{0.11\linewidth}
		\centering {\footnotesize urban 0006}
	\end{minipage} 
	\begin{minipage}[b]{0.11\linewidth}
		\centering {\footnotesize urban 0017}
	\end{minipage} 
	\begin{minipage}[b]{0.11\linewidth}
		\centering {\footnotesize urban 0018}
	\end{minipage} 
	\begin{minipage}[b]{0.11\linewidth}
		\centering {\footnotesize urban 0020}
	\end{minipage} 
	\begin{minipage}[b]{0.11\linewidth}
		\centering {\footnotesize urban 0026}
	\end{minipage} 
	\begin{minipage}[b]{0.11\linewidth}
		\centering {\footnotesize urban 0030}
	\end{minipage} 
	\begin{minipage}[b]{0.11\linewidth}
		\centering {\footnotesize urban 0050}
	\end{minipage} 
	% ------------------------------------------- 
	\caption{Some testing infrared/RGB image pairs. The first row represents the infrared images and the second row represents the corresponding RGB images.}
	\label{Fig:TestIms}
\end{figure*}


%%% double column style.
%%% Training images
%\begin{figure}[th]
%	\centering
%	% ------------------------------------------- 
%%	\begin{minipage}[b]{0.06\linewidth}
%%		\centering
%%		{\footnotesize Infrared} \hfill % \vfill
%%		{\footnotesize RGB}
%%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering
%		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-0.png}
%		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-1.png}
%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering
%		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-2.png}
%		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-3.png}
%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering
%		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-4.png}
%		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-5.png}
%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering
%		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-6.png}
%		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-7.png}
%	\end{minipage} 
%	\\
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering
%		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-8.png}
%		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-9.png}
%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering
%		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-10.png}
%		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-11.png}
%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering
%		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-12.png}
%		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-13.png}
%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering
%		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-14.png}
%		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-15.png}
%	\end{minipage} 
%%	\begin{minipage}[b]{0.24\linewidth}
%%		\centering
%%		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-16.png}
%%		\includegraphics[width = 1.8cm, height = 1.8cm]{./Figures/Dataset/Train_RGB_NIR/train-17.png}
%%	\end{minipage} 
%	\\
%	% ------------------------------------------- 
%	% ------------------------------------------- 
%	%	\begin{minipage}[b]{0.06\linewidth}
%	%		\centering	{\phantom{{\footnotesize Methods}}} 
%	%	\end{minipage}
%	%	\begin{minipage}[b]{0.15\linewidth}
%	%		\centering	{\footnotesize $\sigma=4$}
%	%	\end{minipage} 
%	% -------------------------------------------	
%	\caption{Some training infrared/RGB image pairs.}
%%		 The first row represents the infrared images and the second row represents the corresponding RGB images.}
%	\label{Fig:TrainIms}
%\end{figure}
%%
%%
%%% Testing images
%\begin{figure}[th]
%	\centering
%	% ------------------------------------------- 
%	%	\begin{minipage}[b]{0.06\linewidth}
%	%		\centering
%	%		{\footnotesize Infrared} \hfill % \vfill
%	%		{\footnotesize RGB}
%	%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering
%		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-0.png}
%		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-1.png}
%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering
%		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-2.png}
%		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-3.png}
%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering
%		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-4.png}
%		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-5.png}
%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering
%		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-6.png}
%		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-7.png}
%	\end{minipage} 
%	\\
%	% -------------------------------------------
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering {\footnotesize urban 0004}
%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering {\footnotesize urban 0006}
%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering {\footnotesize urban 0017}
%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering {\footnotesize urban 0018}
%	\end{minipage} 
%	\\
%	\vspace{+0.2cm}
%	% -------------------------------------------
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering
%		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-8.png}
%		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-9.png}
%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering
%		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-10.png}
%		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-11.png}
%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering
%		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-12.png}
%		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-13.png}
%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering
%		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-14.png}
%		\includegraphics[width = 2cm, height = 2cm]{./Figures/Dataset/Test_RGB_NIR/result-15.png}
%	\end{minipage} 
%	\\
%	% ------------------------------------------- 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering {\footnotesize urban 0020}
%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering {\footnotesize urban 0026}
%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering {\footnotesize urban 0030}
%	\end{minipage} 
%	\begin{minipage}[b]{0.24\linewidth}
%		\centering {\footnotesize urban 0050}
%	\end{minipage} 
%	% ------------------------------------------- 
%	\caption{Some testing infrared/RGB image pairs.}
%%		The first row represents the infrared images and the second row represents the corresponding RGB images.}
%	\label{Fig:TestIms}
%\end{figure}
%


%% denoised images for only 3 noise levels
\begin{figure*}[th]
	\begin{multicols}{2}  
		\centering
		% ------------------------------------------- 
		% Noisy images
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Input}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo1_Noise8_X_low.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo1_Noise16_X_low.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo1_Noise24_X_low.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% JBF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize JBF~\cite{kopf2007joint}} % 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo1_Noise8_X_JBF.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo1_Noise16_X_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo1_Noise24_X_JBF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% JBF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap JBF~\cite{kopf2007joint}} % 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo1_Noise8_X_resid_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo1_Noise16_X_resid_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo1_Noise24_X_resid_JBF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% GF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize GF~\cite{he2013guided}}  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo1_Noise8_X_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo1_Noise16_X_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo1_Noise24_X_GF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% GF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap GF~\cite{he2013guided}}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo1_Noise8_X_resid_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo1_Noise16_X_resid_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo1_Noise24_X_resid_GF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% SDF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize SDF~\cite{ham2017robust}} %  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo1_Noise8_X_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo1_Noise16_X_SDF.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo1_Noise24_X_SDF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% SDF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap SDF~\cite{ham2017robust}} % 
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo1_Noise8_X_resid_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo1_Noise16_X_resid_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo1_Noise24_X_resid_SDF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		\begin{minipage}[b]{0.1\linewidth}
			\centering	% {\phantom{{\footnotesize XXX}}} 
		\end{minipage}
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=8$}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=16$} 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=24$} 
		\end{minipage}
		\\
		%---------------------------------------------------
		% true images
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Truth}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo1_Noise8_X_true.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo1_Noise16_X_true.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo1_Noise24_X_true.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% JFSM
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize JFSM\cite{shen2015multispectral}}  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo1_Noise8_X_JFSM.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo1_Noise16_X_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo1_Noise24_X_JFSM.eps}
		\end{minipage} 
		\\
		% -------------------------------------------	
		% JFSM
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap JFSM\cite{shen2015multispectral}}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo1_Noise8_X_resid_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo1_Noise16_X_resid_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo1_Noise24_X_resid_JFSM.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% DJF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize DJF~\cite{li2016deep}} %  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo1_Noise8_X_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo1_Noise16_X_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo1_Noise24_X_DJF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% DJF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap DJF~\cite{li2016deep}} %  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo1_Noise8_X_resid_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo1_Noise16_X_resid_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo1_Noise24_X_resid_DJF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		%	% CDN with standard sparsity
		%	\begin{minipage}[b]{0.1\linewidth}
		%		\centering
		%		{\footnotesize Ours} %  
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo1_Noise4_X_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo1_Noise12_X_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo1_Noise20_X_CDN.eps}
		%	\end{minipage} 
		%	\\
		% -------------------------------------------
		%	% CDN with standard sparsity
		%	\begin{minipage}[b]{0.1\linewidth}
		%		\centering
		%		{\footnotesize ErrMap Ours} %  
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo1_Noise8_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo1_Noise16_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo1_Noise24_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\\
		% -------------------------------------------
		% CDN with group sparsity
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Ours+}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo1_Noise8_X_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo1_Noise16_X_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo1_Noise24_X_CDN.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% CDN with group sparsity
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap Ours+}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo1_Noise8_X_resid_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo1_Noise16_X_resid_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo1_Noise24_X_resid_CDN.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		\begin{minipage}[b]{0.1\linewidth}
			\centering	% {\phantom{{\footnotesize XXX}}} 
		\end{minipage}
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=8$}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=16$} 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=24$} 
		\end{minipage}
		% -------------------------------------------	
	\end{multicols}	

	\vspace{-0.8cm}

	\begin{multicols}{1}  
		\begin{minipage}[b]{0.98\linewidth}
			{\footnotesize Colorbar}
			\includegraphics[width = 16.8cm, height=0.5cm]{./Figures/Colorbar64.eps}
		\end{minipage}
	\end{multicols}	
	
	\vspace{-0.6cm}

	\caption{Visual comparison on multimodal image denoising.}
	%	 Each row represents one approach and its denoising results corresponding to different noise levels.}
	\label{Fig:DenoisedIms_1}
\end{figure*}


%%
%%% error map for only 3 noise levels
%\begin{figure*}[th]
%	\begin{multicols}{2}  
%		\centering
%		% ------------------------------------------- 
%		% JBF
%		\begin{minipage}[b]{0.1\linewidth}
%			\centering
%			{\footnotesize JBF\cite{kopf2007joint}}  
%		\end{minipage} 
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo1_Noise8_X_resid_JBF.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo1_Noise16_X_resid_JBF.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo1_Noise24_X_resid_JBF.eps}
%		\end{minipage} 
%		% ------------------------------------------- 
%		% GF
%		\begin{minipage}[b]{0.1\linewidth}
%			\centering
%			{\footnotesize GF\cite{he2013guided}}  
%		\end{minipage} 
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo1_Noise8_X_resid_GF.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo1_Noise16_X_resid_GF.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo1_Noise24_X_resid_GF.eps}
%		\end{minipage} 
%		% -------------------------------------------
%		% SDF
%		\begin{minipage}[b]{0.1\linewidth}
%			\centering
%			{\footnotesize SDF\cite{ham2017robust}}  
%		\end{minipage}  
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo1_Noise8_X_resid_SDF.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo1_Noise16_X_resid_SDF.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo1_Noise24_X_resid_SDF.eps}
%		\end{minipage} 
%		% -------------------------------------------
%		\begin{minipage}[b]{0.1\linewidth}
%			\centering	% {\phantom{{\footnotesize }}} 
%		\end{minipage}
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering	{\footnotesize $\sigma=8$}
%		\end{minipage} 
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering	{\footnotesize $\sigma=16$} 
%		\end{minipage}  
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering	{\footnotesize $\sigma=24$} 
%		\end{minipage}
%		% -------------------------------------------	
%		% JFSM
%		\begin{minipage}[b]{0.1\linewidth}
%			\centering
%			{\footnotesize JFSM\cite{shen2015multispectral}}  
%		\end{minipage} 
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo1_Noise8_X_resid_JFSM.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo1_Noise16_X_resid_JFSM.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo1_Noise24_X_resid_JFSM.eps}
%		\end{minipage} 
%		% -------------------------------------------
%		% DJF
%		\begin{minipage}[b]{0.1\linewidth}
%			\centering
%			{\footnotesize DJF\cite{li2016deep}} %  
%		\end{minipage}  
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo1_Noise8_X_resid_DJF.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo1_Noise16_X_resid_DJF.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo1_Noise24_X_resid_DJF.eps}
%		\end{minipage} 
%		% -------------------------------------------
%		%	% CDN with standard sparsity
%		%	\begin{minipage}[b]{0.1\linewidth}
%		%		\centering
%		%		{\footnotesize Ours} %  
%		%	\end{minipage} 
%		%	\begin{minipage}[b]{0.28\linewidth}
%		%		\centering
%		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo1_Noise8_X_resid_CDN.eps}
%		%	\end{minipage} 
%		%	\begin{minipage}[b]{0.28\linewidth}
%		%		\centering
%		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo1_Noise16_X_resid_CDN.eps}
%		%	\end{minipage} 
%		%	\begin{minipage}[b]{0.28\linewidth}
%		%		\centering
%		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo1_Noise24_X_resid_CDN.eps}
%		%	\end{minipage} 
%		% -------------------------------------------
%		% CDN with group sparsity
%		\begin{minipage}[b]{0.1\linewidth}
%			\centering
%			{\footnotesize Ours+}  
%		\end{minipage} 
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo1_Noise8_X_resid_CDN.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo1_Noise16_X_resid_CDN.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo1_Noise24_X_resid_CDN.eps}
%		\end{minipage} 
%		%---------------------------------------------------
%		\begin{minipage}[b]{0.1\linewidth}
%			\centering	% {\phantom{{\footnotesize }}} 
%		\end{minipage}
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering	{\footnotesize $\sigma=8$}
%		\end{minipage} 
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering	{\footnotesize $\sigma=16$} 
%		\end{minipage}  
%		\begin{minipage}[b]{0.28\linewidth}
%			\centering	{\footnotesize $\sigma=24$} 
%		\end{minipage}
%		% -------------------------------------------	
%	\end{multicols}
%	\caption{Visual comparison on the error maps for multimodal image denoising.}
%	\label{Fig:Residual}
%\end{figure*}




%% image No2 -- denoised images for only 3 noise levels
\begin{figure*}[th]
	\begin{multicols}{2}  
		\centering
		% ------------------------------------------- 
		% Noisy images
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Input}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo2_Noise8_X_low.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo2_Noise16_X_low.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo2_Noise24_X_low.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% JBF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize JBF~\cite{kopf2007joint}} % 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo2_Noise8_X_JBF.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo2_Noise16_X_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo2_Noise24_X_JBF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% JBF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap JBF~\cite{kopf2007joint}} % 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo2_Noise8_X_resid_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo2_Noise16_X_resid_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo2_Noise24_X_resid_JBF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% GF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize GF~\cite{he2013guided}}  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo2_Noise8_X_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo2_Noise16_X_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo2_Noise24_X_GF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% GF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap GF~\cite{he2013guided}}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo2_Noise8_X_resid_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo2_Noise16_X_resid_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo2_Noise24_X_resid_GF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% SDF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize SDF~\cite{ham2017robust}} %  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo2_Noise8_X_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo2_Noise16_X_SDF.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo2_Noise24_X_SDF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% SDF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap SDF~\cite{ham2017robust}} % 
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo2_Noise8_X_resid_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo2_Noise16_X_resid_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo2_Noise24_X_resid_SDF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		\begin{minipage}[b]{0.1\linewidth}
			\centering	% {\phantom{{\footnotesize XXX}}} 
		\end{minipage}
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=8$}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=16$} 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=24$} 
		\end{minipage}
		\\
		%---------------------------------------------------
		% true images
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Truth}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo2_Noise8_X_true.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo2_Noise16_X_true.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo2_Noise24_X_true.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% JFSM
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize JFSM\cite{shen2015multispectral}}  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo2_Noise8_X_JFSM.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo2_Noise16_X_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo2_Noise24_X_JFSM.eps}
		\end{minipage} 
		\\
		% -------------------------------------------	
		% JFSM
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap JFSM\cite{shen2015multispectral}}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo2_Noise8_X_resid_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo2_Noise16_X_resid_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo2_Noise24_X_resid_JFSM.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% DJF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize DJF~\cite{li2016deep}} %  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo2_Noise8_X_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo2_Noise16_X_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo2_Noise24_X_DJF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% DJF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap DJF~\cite{li2016deep}} %  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo2_Noise8_X_resid_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo2_Noise16_X_resid_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo2_Noise24_X_resid_DJF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		%	% CDN with standard sparsity
		%	\begin{minipage}[b]{0.1\linewidth}
		%		\centering
		%		{\footnotesize Ours} %  
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo2_Noise4_X_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo2_Noise12_X_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo2_Noise20_X_CDN.eps}
		%	\end{minipage} 
		%	\\
		% -------------------------------------------
		%	% CDN with standard sparsity
		%	\begin{minipage}[b]{0.1\linewidth}
		%		\centering
		%		{\footnotesize ErrMap Ours} %  
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo2_Noise8_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo2_Noise16_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo2_Noise24_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\\
		% -------------------------------------------
		% CDN with group sparsity
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Ours+}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo2_Noise8_X_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo2_Noise16_X_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo2_Noise24_X_CDN.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% CDN with group sparsity
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap Ours+}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo2_Noise8_X_resid_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo2_Noise16_X_resid_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo2_Noise24_X_resid_CDN.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		\begin{minipage}[b]{0.1\linewidth}
			\centering	% {\phantom{{\footnotesize XXX}}} 
		\end{minipage}
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=8$}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=16$} 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=24$} 
		\end{minipage}
		% -------------------------------------------	
	\end{multicols}	
	
	\vspace{-0.8cm}
	
	\begin{multicols}{1}  
		\begin{minipage}[b]{0.98\linewidth}
			{\footnotesize Colorbar}
			\includegraphics[width = 16.8cm, height=0.5cm]{./Figures/Colorbar64.eps}
		\end{minipage}
	\end{multicols}	
	
	\vspace{-0.6cm}
	
	\caption{Visual comparison on multimodal image denoising.}
	%	 Each row represents one approach and its denoising results corresponding to different noise levels.}
	\label{Fig:DenoisedIms_2}
\end{figure*}




%%=====================================================================================







%% image No3 -- denoised images for only 3 noise levels
\begin{figure*}[th]
	\begin{multicols}{2}  
		\centering
		% ------------------------------------------- 
		% Noisy images
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Input}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo3_Noise8_X_low.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo3_Noise16_X_low.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo3_Noise24_X_low.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% JBF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize JBF~\cite{kopf2007joint}} % 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo3_Noise8_X_JBF.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo3_Noise16_X_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo3_Noise24_X_JBF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% JBF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap JBF~\cite{kopf2007joint}} % 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo3_Noise8_X_resid_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo3_Noise16_X_resid_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo3_Noise24_X_resid_JBF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% GF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize GF~\cite{he2013guided}}  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo3_Noise8_X_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo3_Noise16_X_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo3_Noise24_X_GF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% GF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap GF~\cite{he2013guided}}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo3_Noise8_X_resid_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo3_Noise16_X_resid_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo3_Noise24_X_resid_GF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% SDF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize SDF~\cite{ham2017robust}} %  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo3_Noise8_X_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo3_Noise16_X_SDF.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo3_Noise24_X_SDF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% SDF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap SDF~\cite{ham2017robust}} % 
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo3_Noise8_X_resid_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo3_Noise16_X_resid_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo3_Noise24_X_resid_SDF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		\begin{minipage}[b]{0.1\linewidth}
			\centering	% {\phantom{{\footnotesize XXX}}} 
		\end{minipage}
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=8$}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=16$} 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=24$} 
		\end{minipage}
		\\
		%---------------------------------------------------
		% true images
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Truth}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo3_Noise8_X_true.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo3_Noise16_X_true.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo3_Noise24_X_true.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% JFSM
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize JFSM\cite{shen2015multispectral}}  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo3_Noise8_X_JFSM.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo3_Noise16_X_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo3_Noise24_X_JFSM.eps}
		\end{minipage} 
		\\
		% -------------------------------------------	
		% JFSM
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap JFSM\cite{shen2015multispectral}}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo3_Noise8_X_resid_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo3_Noise16_X_resid_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo3_Noise24_X_resid_JFSM.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% DJF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize DJF~\cite{li2016deep}} %  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo3_Noise8_X_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo3_Noise16_X_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo3_Noise24_X_DJF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% DJF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap DJF~\cite{li2016deep}} %  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo3_Noise8_X_resid_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo3_Noise16_X_resid_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo3_Noise24_X_resid_DJF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		%	% CDN with standard sparsity
		%	\begin{minipage}[b]{0.1\linewidth}
		%		\centering
		%		{\footnotesize Ours} %  
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo3_Noise4_X_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo3_Noise12_X_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo3_Noise20_X_CDN.eps}
		%	\end{minipage} 
		%	\\
		% -------------------------------------------
		%	% CDN with standard sparsity
		%	\begin{minipage}[b]{0.1\linewidth}
		%		\centering
		%		{\footnotesize ErrMap Ours} %  
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo3_Noise8_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo3_Noise16_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo3_Noise24_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\\
		% -------------------------------------------
		% CDN with group sparsity
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Ours+}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo3_Noise8_X_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo3_Noise16_X_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo3_Noise24_X_CDN.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% CDN with group sparsity
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap Ours+}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo3_Noise8_X_resid_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo3_Noise16_X_resid_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo3_Noise24_X_resid_CDN.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		\begin{minipage}[b]{0.1\linewidth}
			\centering	% {\phantom{{\footnotesize XXX}}} 
		\end{minipage}
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=8$}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=16$} 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=24$} 
		\end{minipage}
		% -------------------------------------------	
	\end{multicols}	
	
	\vspace{-0.8cm}
	
	\begin{multicols}{1}  
		\begin{minipage}[b]{0.98\linewidth}
			{\footnotesize Colorbar}
			\includegraphics[width = 16.8cm, height=0.5cm]{./Figures/Colorbar64.eps}
		\end{minipage}
	\end{multicols}	
	
	\vspace{-0.6cm}
	
	\caption{Visual comparison on multimodal image denoising.}
	%	 Each row represents one approach and its denoising results corresponding to different noise levels.}
	\label{Fig:DenoisedIms_3}
\end{figure*}





%%======================================================================================





%% image No4 -- denoised images for only 3 noise levels
\begin{figure*}[th]
	\begin{multicols}{2}  
		\centering
		% ------------------------------------------- 
		% Noisy images
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Input}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo4_Noise8_X_low.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo4_Noise16_X_low.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo4_Noise24_X_low.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% JBF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize JBF~\cite{kopf2007joint}} % 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo4_Noise8_X_JBF.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo4_Noise16_X_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo4_Noise24_X_JBF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% JBF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap JBF~\cite{kopf2007joint}} % 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo4_Noise8_X_resid_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo4_Noise16_X_resid_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo4_Noise24_X_resid_JBF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% GF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize GF~\cite{he2013guided}}  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo4_Noise8_X_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo4_Noise16_X_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo4_Noise24_X_GF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% GF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap GF~\cite{he2013guided}}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo4_Noise8_X_resid_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo4_Noise16_X_resid_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo4_Noise24_X_resid_GF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% SDF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize SDF~\cite{ham2017robust}} %  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo4_Noise8_X_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo4_Noise16_X_SDF.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo4_Noise24_X_SDF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% SDF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap SDF~\cite{ham2017robust}} % 
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo4_Noise8_X_resid_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo4_Noise16_X_resid_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo4_Noise24_X_resid_SDF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		\begin{minipage}[b]{0.1\linewidth}
			\centering	% {\phantom{{\footnotesize XXX}}} 
		\end{minipage}
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=8$}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=16$} 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=24$} 
		\end{minipage}
		\\
		%---------------------------------------------------
		% true images
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Truth}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo4_Noise8_X_true.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo4_Noise16_X_true.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo4_Noise24_X_true.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% JFSM
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize JFSM\cite{shen2015multispectral}}  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo4_Noise8_X_JFSM.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo4_Noise16_X_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo4_Noise24_X_JFSM.eps}
		\end{minipage} 
		\\
		% -------------------------------------------	
		% JFSM
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap JFSM\cite{shen2015multispectral}}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo4_Noise8_X_resid_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo4_Noise16_X_resid_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo4_Noise24_X_resid_JFSM.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% DJF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize DJF~\cite{li2016deep}} %  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo4_Noise8_X_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo4_Noise16_X_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo4_Noise24_X_DJF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% DJF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap DJF~\cite{li2016deep}} %  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo4_Noise8_X_resid_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo4_Noise16_X_resid_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo4_Noise24_X_resid_DJF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		%	% CDN with standard sparsity
		%	\begin{minipage}[b]{0.1\linewidth}
		%		\centering
		%		{\footnotesize Ours} %  
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo4_Noise4_X_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo4_Noise12_X_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo4_Noise20_X_CDN.eps}
		%	\end{minipage} 
		%	\\
		% -------------------------------------------
		%	% CDN with standard sparsity
		%	\begin{minipage}[b]{0.1\linewidth}
		%		\centering
		%		{\footnotesize ErrMap Ours} %  
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo4_Noise8_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo4_Noise16_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo4_Noise24_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\\
		% -------------------------------------------
		% CDN with group sparsity
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Ours+}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo4_Noise8_X_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo4_Noise16_X_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo4_Noise24_X_CDN.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% CDN with group sparsity
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap Ours+}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo4_Noise8_X_resid_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo4_Noise16_X_resid_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo4_Noise24_X_resid_CDN.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		\begin{minipage}[b]{0.1\linewidth}
			\centering	% {\phantom{{\footnotesize XXX}}} 
		\end{minipage}
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=8$}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=16$} 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=24$} 
		\end{minipage}
		% -------------------------------------------	
	\end{multicols}	
	
	\vspace{-0.8cm}
	
	\begin{multicols}{1}  
		\begin{minipage}[b]{0.98\linewidth}
			{\footnotesize Colorbar}
			\includegraphics[width = 16.8cm, height=0.5cm]{./Figures/Colorbar64.eps}
		\end{minipage}
	\end{multicols}	
	
	\vspace{-0.6cm}
	
	\caption{Visual comparison on multimodal image denoising.}
	%	 Each row represents one approach and its denoising results corresponding to different noise levels.}
	\label{Fig:DenoisedIms_4}
\end{figure*}



%%==========================================================================================





%% image No5 -- denoised images for only 3 noise levels
\begin{figure*}[th]
	\begin{multicols}{2}  
		\centering
		% ------------------------------------------- 
		% Noisy images
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Input}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo5_Noise8_X_low.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo5_Noise16_X_low.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo5_Noise24_X_low.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% JBF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize JBF~\cite{kopf2007joint}} % 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo5_Noise8_X_JBF.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo5_Noise16_X_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo5_Noise24_X_JBF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% JBF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap JBF~\cite{kopf2007joint}} % 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo5_Noise8_X_resid_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo5_Noise16_X_resid_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo5_Noise24_X_resid_JBF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% GF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize GF~\cite{he2013guided}}  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo5_Noise8_X_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo5_Noise16_X_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo5_Noise24_X_GF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% GF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap GF~\cite{he2013guided}}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo5_Noise8_X_resid_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo5_Noise16_X_resid_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo5_Noise24_X_resid_GF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% SDF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize SDF~\cite{ham2017robust}} %  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo5_Noise8_X_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo5_Noise16_X_SDF.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo5_Noise24_X_SDF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% SDF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap SDF~\cite{ham2017robust}} % 
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo5_Noise8_X_resid_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo5_Noise16_X_resid_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo5_Noise24_X_resid_SDF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		\begin{minipage}[b]{0.1\linewidth}
			\centering	% {\phantom{{\footnotesize XXX}}} 
		\end{minipage}
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=8$}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=16$} 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=24$} 
		\end{minipage}
		\\
		%---------------------------------------------------
		% true images
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Truth}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo5_Noise8_X_true.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo5_Noise16_X_true.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo5_Noise24_X_true.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% JFSM
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize JFSM\cite{shen2015multispectral}}  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo5_Noise8_X_JFSM.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo5_Noise16_X_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo5_Noise24_X_JFSM.eps}
		\end{minipage} 
		\\
		% -------------------------------------------	
		% JFSM
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap JFSM\cite{shen2015multispectral}}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo5_Noise8_X_resid_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo5_Noise16_X_resid_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo5_Noise24_X_resid_JFSM.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% DJF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize DJF~\cite{li2016deep}} %  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo5_Noise8_X_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo5_Noise16_X_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo5_Noise24_X_DJF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% DJF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap DJF~\cite{li2016deep}} %  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo5_Noise8_X_resid_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo5_Noise16_X_resid_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo5_Noise24_X_resid_DJF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		%	% CDN with standard sparsity
		%	\begin{minipage}[b]{0.1\linewidth}
		%		\centering
		%		{\footnotesize Ours} %  
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo5_Noise4_X_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo5_Noise12_X_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo5_Noise20_X_CDN.eps}
		%	\end{minipage} 
		%	\\
		% -------------------------------------------
		%	% CDN with standard sparsity
		%	\begin{minipage}[b]{0.1\linewidth}
		%		\centering
		%		{\footnotesize ErrMap Ours} %  
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo5_Noise8_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo5_Noise16_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo5_Noise24_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\\
		% -------------------------------------------
		% CDN with group sparsity
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Ours+}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo5_Noise8_X_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo5_Noise16_X_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo5_Noise24_X_CDN.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% CDN with group sparsity
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap Ours+}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo5_Noise8_X_resid_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo5_Noise16_X_resid_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo5_Noise24_X_resid_CDN.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		\begin{minipage}[b]{0.1\linewidth}
			\centering	% {\phantom{{\footnotesize XXX}}} 
		\end{minipage}
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=8$}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=16$} 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=24$} 
		\end{minipage}
		% -------------------------------------------	
	\end{multicols}	
	
	\vspace{-0.8cm}
	
	\begin{multicols}{1}  
		\begin{minipage}[b]{0.98\linewidth}
			{\footnotesize Colorbar}
			\includegraphics[width = 16.8cm, height=0.5cm]{./Figures/Colorbar64.eps}
		\end{minipage}
	\end{multicols}	
	
	\vspace{-0.6cm}
	
	\caption{Visual comparison on multimodal image denoising.}
	%	 Each row represents one approach and its denoising results corresponding to different noise levels.}
	\label{Fig:DenoisedIms_5}
\end{figure*}



%%================================================================================================








%% image No6 -- denoised images for only 3 noise levels
\begin{figure*}[th]
	\begin{multicols}{2}  
		\centering
		% ------------------------------------------- 
		% Noisy images
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Input}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo6_Noise8_X_low.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo6_Noise16_X_low.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo6_Noise24_X_low.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% JBF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize JBF~\cite{kopf2007joint}} % 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo6_Noise8_X_JBF.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo6_Noise16_X_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo6_Noise24_X_JBF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% JBF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap JBF~\cite{kopf2007joint}} % 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo6_Noise8_X_resid_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo6_Noise16_X_resid_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo6_Noise24_X_resid_JBF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% GF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize GF~\cite{he2013guided}}  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo6_Noise8_X_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo6_Noise16_X_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo6_Noise24_X_GF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% GF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap GF~\cite{he2013guided}}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo6_Noise8_X_resid_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo6_Noise16_X_resid_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo6_Noise24_X_resid_GF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% SDF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize SDF~\cite{ham2017robust}} %  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo6_Noise8_X_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo6_Noise16_X_SDF.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo6_Noise24_X_SDF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% SDF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap SDF~\cite{ham2017robust}} % 
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo6_Noise8_X_resid_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo6_Noise16_X_resid_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo6_Noise24_X_resid_SDF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		\begin{minipage}[b]{0.1\linewidth}
			\centering	% {\phantom{{\footnotesize XXX}}} 
		\end{minipage}
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=8$}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=16$} 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=24$} 
		\end{minipage}
		\\
		%---------------------------------------------------
		% true images
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Truth}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo6_Noise8_X_true.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo6_Noise16_X_true.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo6_Noise24_X_true.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% JFSM
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize JFSM\cite{shen2015multispectral}}  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo6_Noise8_X_JFSM.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo6_Noise16_X_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo6_Noise24_X_JFSM.eps}
		\end{minipage} 
		\\
		% -------------------------------------------	
		% JFSM
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap JFSM\cite{shen2015multispectral}}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo6_Noise8_X_resid_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo6_Noise16_X_resid_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo6_Noise24_X_resid_JFSM.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% DJF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize DJF~\cite{li2016deep}} %  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo6_Noise8_X_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo6_Noise16_X_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo6_Noise24_X_DJF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% DJF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap DJF~\cite{li2016deep}} %  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo6_Noise8_X_resid_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo6_Noise16_X_resid_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo6_Noise24_X_resid_DJF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		%	% CDN with standard sparsity
		%	\begin{minipage}[b]{0.1\linewidth}
		%		\centering
		%		{\footnotesize Ours} %  
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo6_Noise4_X_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo6_Noise12_X_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo6_Noise20_X_CDN.eps}
		%	\end{minipage} 
		%	\\
		% -------------------------------------------
		%	% CDN with standard sparsity
		%	\begin{minipage}[b]{0.1\linewidth}
		%		\centering
		%		{\footnotesize ErrMap Ours} %  
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo6_Noise8_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo6_Noise16_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo6_Noise24_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\\
		% -------------------------------------------
		% CDN with group sparsity
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Ours+}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo6_Noise8_X_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo6_Noise16_X_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo6_Noise24_X_CDN.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% CDN with group sparsity
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap Ours+}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo6_Noise8_X_resid_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo6_Noise16_X_resid_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo6_Noise24_X_resid_CDN.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		\begin{minipage}[b]{0.1\linewidth}
			\centering	% {\phantom{{\footnotesize XXX}}} 
		\end{minipage}
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=8$}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=16$} 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=24$} 
		\end{minipage}
		% -------------------------------------------	
	\end{multicols}	
	
	\vspace{-0.8cm}
	
	\begin{multicols}{1}  
		\begin{minipage}[b]{0.98\linewidth}
			{\footnotesize Colorbar}
			\includegraphics[width = 16.8cm, height=0.5cm]{./Figures/Colorbar64.eps}
		\end{minipage}
	\end{multicols}	
	
	\vspace{-0.6cm}
	
	\caption{Visual comparison on multimodal image denoising.}
	%	 Each row represents one approach and its denoising results corresponding to different noise levels.}
	\label{Fig:DenoisedIms_6}
\end{figure*}


%%=====================================================================================





%% image No7 -- denoised images for only 3 noise levels
\begin{figure*}[th]
	\begin{multicols}{2}  
		\centering
		% ------------------------------------------- 
		% Noisy images
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Input}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo7_Noise8_X_low.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo7_Noise16_X_low.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo7_Noise24_X_low.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% JBF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize JBF~\cite{kopf2007joint}} % 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo7_Noise8_X_JBF.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo7_Noise16_X_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo7_Noise24_X_JBF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% JBF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap JBF~\cite{kopf2007joint}} % 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo7_Noise8_X_resid_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo7_Noise16_X_resid_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo7_Noise24_X_resid_JBF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% GF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize GF~\cite{he2013guided}}  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo7_Noise8_X_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo7_Noise16_X_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo7_Noise24_X_GF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% GF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap GF~\cite{he2013guided}}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo7_Noise8_X_resid_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo7_Noise16_X_resid_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo7_Noise24_X_resid_GF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% SDF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize SDF~\cite{ham2017robust}} %  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo7_Noise8_X_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo7_Noise16_X_SDF.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo7_Noise24_X_SDF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% SDF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap SDF~\cite{ham2017robust}} % 
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo7_Noise8_X_resid_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo7_Noise16_X_resid_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo7_Noise24_X_resid_SDF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		\begin{minipage}[b]{0.1\linewidth}
			\centering	% {\phantom{{\footnotesize XXX}}} 
		\end{minipage}
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=8$}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=16$} 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=24$} 
		\end{minipage}
		\\
		%---------------------------------------------------
		% true images
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Truth}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo7_Noise8_X_true.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo7_Noise16_X_true.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo7_Noise24_X_true.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% JFSM
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize JFSM\cite{shen2015multispectral}}  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo7_Noise8_X_JFSM.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo7_Noise16_X_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo7_Noise24_X_JFSM.eps}
		\end{minipage} 
		\\
		% -------------------------------------------	
		% JFSM
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap JFSM\cite{shen2015multispectral}}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo7_Noise8_X_resid_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo7_Noise16_X_resid_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo7_Noise24_X_resid_JFSM.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% DJF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize DJF~\cite{li2016deep}} %  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo7_Noise8_X_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo7_Noise16_X_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo7_Noise24_X_DJF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% DJF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap DJF~\cite{li2016deep}} %  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo7_Noise8_X_resid_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo7_Noise16_X_resid_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo7_Noise24_X_resid_DJF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		%	% CDN with standard sparsity
		%	\begin{minipage}[b]{0.1\linewidth}
		%		\centering
		%		{\footnotesize Ours} %  
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo7_Noise4_X_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo7_Noise12_X_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo7_Noise20_X_CDN.eps}
		%	\end{minipage} 
		%	\\
		% -------------------------------------------
		%	% CDN with standard sparsity
		%	\begin{minipage}[b]{0.1\linewidth}
		%		\centering
		%		{\footnotesize ErrMap Ours} %  
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo7_Noise8_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo7_Noise16_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo7_Noise24_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\\
		% -------------------------------------------
		% CDN with group sparsity
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Ours+}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo7_Noise8_X_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo7_Noise16_X_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo7_Noise24_X_CDN.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% CDN with group sparsity
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap Ours+}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo7_Noise8_X_resid_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo7_Noise16_X_resid_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo7_Noise24_X_resid_CDN.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		\begin{minipage}[b]{0.1\linewidth}
			\centering	% {\phantom{{\footnotesize XXX}}} 
		\end{minipage}
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=8$}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=16$} 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=24$} 
		\end{minipage}
		% -------------------------------------------	
	\end{multicols}	
	
	\vspace{-0.8cm}
	
	\begin{multicols}{1}  
		\begin{minipage}[b]{0.98\linewidth}
			{\footnotesize Colorbar}
			\includegraphics[width = 16.8cm, height=0.5cm]{./Figures/Colorbar64.eps}
		\end{minipage}
	\end{multicols}	
	
	\vspace{-0.6cm}
	
	\caption{Visual comparison on multimodal image denoising.}
	%	 Each row represents one approach and its denoising results corresponding to different noise levels.}
	\label{Fig:DenoisedIms_7}
\end{figure*}



%%========================================================================================




%% image No8 -- denoised images for only 3 noise levels
\begin{figure*}[th]
	\begin{multicols}{2}  
		\centering
		% ------------------------------------------- 
		% Noisy images
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Input}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo8_Noise8_X_low.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo8_Noise16_X_low.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo8_Noise24_X_low.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% JBF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize JBF~\cite{kopf2007joint}} % 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo8_Noise8_X_JBF.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo8_Noise16_X_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo8_Noise24_X_JBF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% JBF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap JBF~\cite{kopf2007joint}} % 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo8_Noise8_X_resid_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo8_Noise16_X_resid_JBF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JBF/ImgNo8_Noise24_X_resid_JBF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% GF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize GF~\cite{he2013guided}}  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo8_Noise8_X_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo8_Noise16_X_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo8_Noise24_X_GF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		% GF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap GF~\cite{he2013guided}}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo8_Noise8_X_resid_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo8_Noise16_X_resid_GF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo8_Noise24_X_resid_GF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% SDF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize SDF~\cite{ham2017robust}} %  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo8_Noise8_X_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo8_Noise16_X_SDF.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo8_Noise24_X_SDF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% SDF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap SDF~\cite{ham2017robust}} % 
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo8_Noise8_X_resid_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo8_Noise16_X_resid_SDF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/SDF/ImgNo8_Noise24_X_resid_SDF.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		\begin{minipage}[b]{0.1\linewidth}
			\centering	% {\phantom{{\footnotesize XXX}}} 
		\end{minipage}
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=8$}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=16$} 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=24$} 
		\end{minipage}
		\\
		%---------------------------------------------------
		% true images
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Truth}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo8_Noise8_X_true.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo8_Noise16_X_true.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/GF/ImgNo8_Noise24_X_true.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% JFSM
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize JFSM\cite{shen2015multispectral}}  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo8_Noise8_X_JFSM.eps}
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo8_Noise16_X_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo8_Noise24_X_JFSM.eps}
		\end{minipage} 
		\\
		% -------------------------------------------	
		% JFSM
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap JFSM\cite{shen2015multispectral}}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo8_Noise8_X_resid_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo8_Noise16_X_resid_JFSM.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/JFSM/ImgNo8_Noise24_X_resid_JFSM.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% DJF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize DJF~\cite{li2016deep}} %  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo8_Noise8_X_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo8_Noise16_X_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo8_Noise24_X_DJF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% DJF
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap DJF~\cite{li2016deep}} %  
		\end{minipage}  
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo8_Noise8_X_resid_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo8_Noise16_X_resid_DJF.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/DJF/ImgNo8_Noise24_X_resid_DJF.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		%	% CDN with standard sparsity
		%	\begin{minipage}[b]{0.1\linewidth}
		%		\centering
		%		{\footnotesize Ours} %  
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo8_Noise4_X_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo8_Noise12_X_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo8_Noise20_X_CDN.eps}
		%	\end{minipage} 
		%	\\
		% -------------------------------------------
		%	% CDN with standard sparsity
		%	\begin{minipage}[b]{0.1\linewidth}
		%		\centering
		%		{\footnotesize ErrMap Ours} %  
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo8_Noise8_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo8_Noise16_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\begin{minipage}[b]{0.28\linewidth}
		%		\centering
		%		\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN/ImgNo8_Noise24_X_resid_CDN.eps}
		%	\end{minipage} 
		%	\\
		% -------------------------------------------
		% CDN with group sparsity
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize Ours+}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo8_Noise8_X_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo8_Noise16_X_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo8_Noise24_X_CDN.eps}
		\end{minipage} 
		\\
		% -------------------------------------------
		% CDN with group sparsity
		\begin{minipage}[b]{0.1\linewidth}
			\centering
			{\footnotesize ErrMap Ours+}  
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo8_Noise8_X_resid_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo8_Noise16_X_resid_CDN.eps}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering
			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_GrpSp/ImgNo8_Noise24_X_resid_CDN.eps}
		\end{minipage} 
		\\
		% ------------------------------------------- 
		\begin{minipage}[b]{0.1\linewidth}
			\centering	% {\phantom{{\footnotesize XXX}}} 
		\end{minipage}
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=8$}
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=16$} 
		\end{minipage} 
		\begin{minipage}[b]{0.28\linewidth}
			\centering	{\footnotesize $\sigma=24$} 
		\end{minipage}
		% -------------------------------------------	
	\end{multicols}	
	
	\vspace{-0.8cm}
	
	\begin{multicols}{1}  
		\begin{minipage}[b]{0.98\linewidth}
			{\footnotesize Colorbar}
			\includegraphics[width = 16.8cm, height=0.5cm]{./Figures/Colorbar64.eps}
		\end{minipage}
	\end{multicols}	
	
	\vspace{-0.6cm}
	
	\caption{Visual comparison on multimodal image denoising.}
	%	 Each row represents one approach and its denoising results corresponding to different noise levels.}
	\label{Fig:DenoisedIms_8}
\end{figure*}





%
%%% denoised images figures 1 - 8
%\begin{figure*}[t]
%	\begin{multicols}{2}  
%		\centering
%		% ------------------------------------------- 
%		% Noisy input, Denoised image, truth
%		\begin{minipage}[b]{0.06\linewidth}
%			\centering
%			{\footnotesize urban 0004}  
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo1_Noise24_X_low.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo1_Noise24_X_CDN.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo1_Noise24_X_true.eps}
%		\end{minipage} 
%		\\
%		% ------------------------------------------- 
%		% Noisy input, Denoised image, truth
%		\begin{minipage}[b]{0.06\linewidth}
%			\centering
%			{\footnotesize urban 0006}  
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo2_Noise24_X_low.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo2_Noise24_X_CDN.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo2_Noise24_X_true.eps}
%		\end{minipage} 
%		\\
%		% ------------------------------------------- 
%		% Noisy input, Denoised image, truth
%		\begin{minipage}[b]{0.06\linewidth}
%			\centering
%			{\footnotesize urban 0017}  
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo3_Noise24_X_low.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo3_Noise24_X_CDN.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo3_Noise24_X_true.eps}
%		\end{minipage} 
%		\\
%		% ------------------------------------------- 
%		% Noisy input, Denoised image, truth
%		\begin{minipage}[b]{0.06\linewidth}
%			\centering
%			{\footnotesize urban 0018}  
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo4_Noise24_X_low.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo4_Noise24_X_CDN.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo4_Noise24_X_true.eps}
%		\end{minipage} 
%		\\
%		% -------------------------------------------  
%		\begin{minipage}[b]{0.06\linewidth}
%			\centering	% {\phantom{{\footnotesize XXX}}} 
%		\end{minipage}
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering	{\footnotesize Noisy Input}
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering	{\footnotesize Denoised} 
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering	{\footnotesize Groundtruth} 
%		\end{minipage}
%		\\
%		% ------------------------------------------- 
%		% Noisy input, Denoised image, truth
%		\begin{minipage}[b]{0.06\linewidth}
%			\centering
%			{\footnotesize urban 0020}  
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo5_Noise24_X_low.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo5_Noise24_X_CDN.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo5_Noise24_X_true.eps}
%		\end{minipage} 
%		\\
%		% ------------------------------------------- 
%		% Noisy input, Denoised image, truth
%		\begin{minipage}[b]{0.06\linewidth}
%			\centering
%			{\footnotesize urban 0026}  
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo6_Noise24_X_low.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo6_Noise24_X_CDN.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo6_Noise24_X_true.eps}
%		\end{minipage} 
%		\\
%		% ------------------------------------------- 
%		% Noisy input, Denoised image, truth
%		\begin{minipage}[b]{0.06\linewidth}
%			\centering
%			{\footnotesize urban 0030}  
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo7_Noise24_X_low.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo7_Noise24_X_CDN.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo7_Noise24_X_true.eps}
%		\end{minipage} 
%		\\
%		% ------------------------------------------- 
%		% Noisy input, Denoised image, truth
%		\begin{minipage}[b]{0.06\linewidth}
%			\centering
%			{\footnotesize urban 0050}  
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo8_Noise24_X_low.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo8_Noise24_X_CDN.eps}
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering
%			\includegraphics[width = 2.5cm, height = 2.5cm]{./Figures/CDN_Figures1-8_Noise24/ImgNo8_Noise24_X_true.eps}
%		\end{minipage} 
%		\\
%		% ------------------------------------------- 
%		\begin{minipage}[b]{0.06\linewidth}
%			\centering	% {\phantom{{\footnotesize XXX}}} 
%		\end{minipage}
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering	{\footnotesize Noisy Input}
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering	{\footnotesize Denoised} 
%		\end{minipage} 
%		\begin{minipage}[b]{0.3\linewidth}
%			\centering	{\footnotesize Groundtruth} 
%		\end{minipage}
%		% -------------------------------------------
%	\end{multicols}	
%	\caption{Multimodal image denoising results of our algorithm with group sparsity regularization at $\sigma = 24$.}
%	\label{Fig:DenoisedIms_CDN}
%\end{figure*}







